Arithmetic Transformers Can Length-Generalize in Both Operand Length and Count

Transformers often struggle with length generalization, meaning they fail to generalize to sequences longer than those encountered during training. While arithmetic tasks are commonly used to study length generalization, certain tasks are considered notoriously difficult, e.g., multi-operand addition (requiring generalization over both the number of operands and their lengths) and multiplication (requiring generalization over both operand lengths). In this work, we achieve approximately 2-3x length generalization on both tasks, which is the first such achievement in arithmetic Transformers. We design task-specific scratchpads enabling the model to focus on a fixed number of tokens per each next-token prediction step, and apply multi-level versions of \Position Coupling (Cho et al., 2024; McLeish et al., 2024) to let Transformers know the right position to attend to. On the theory side, we prove that a 1-layer Transformer using our method can solve multi-operand addition, up to operand length and operand count that are exponential in embedding dimension.

==> Figure/code/addition_method_compare.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{Figure/addition_method_compare.pdf}
    \caption{\textbf{Comparison of methods in the integer addition task.} We report exact-match accuracies for the addition task, with results taken as the median over 4 seeds for each method (6 seeds for our approach). The x-axis corresponds to the number of operands, and the y-axis indicates the maximum digit length of operands. The red box indicates the training distribution, $\gS_A(10, 10)$. \textcolor{red}{need to refine the figure}}
    \label{fig:addition_method_compare}
\end{figure}

==> Figure/code/addition_onlyanswer.tex <==
\begin{figure}[H]
    \centering
    % \includegraphics[width=1\linewidth]{Figure/addition_architecture.pdf}
    \includegraphics[width=1\linewidth]{Figure/MultiAdd_Inputformats_Ans.pdf}
    \caption{\fix{\textbf{Comparison of the input formats in the integer addition task.} We report exact-match accuracies for the addition task, with results taken as the median over 8 seeds for each configuration. In this figure, predictions are considered correct if the final answer is correct, regardless of the scratchpad. The x-axis corresponds to the number of operands, and the y-axis indicates the length of operands. The red box indicates the trained scope $\gS_A(10,10)$.}}
    \label{fig:addition_onlyanswer}
\end{figure}
